Global well-posedness of the dynamical sine-Gordon model up to $6\pi$

We prove the global well-posedness of the dynamical sine-Gordon model up to the third threshold, i.e., for parameters $\beta^2 < 6\pi$. The key novelty in our approach is the introduction of the so-called resonant equation, whose solution is entirely deterministic and completely captures the size of the solution to the dynamical sine-Gordon model. The probabilistic fluctuations in the dynamical sine-Gordon model are then controlled using uniform estimates for modified stochastic objects.

==> scratch.tex <==
% \sky{Not sure if we should provide more detail about this. I think there is a soft argument as follows. Abstractly, there are measurable functions $F_\varep, F$ such that $u_\varep = F_\varep(\zeta_{[t_0 - \varep, \infty)})$, and $u = F(\zeta_{[t_0, \infty)}, \mc{N})$, where $\mc{N}$ is the set of null sets of our probability space. For the latter, we use that $u$ is measurable with respect to $\bigcap_{\varep > 0}\sigma(\zeta |_{[t_0 - \varep, \infty)})$, and then left continuity to say that this is equal to the sigma algebra $\sigma(\zeta_{[t_0, \infty)} \cup \mc{N})$ (here we use that the completion of the natural filtration of Brownian motion is right continuous). Then by some abstract measure theory, we have that if a random variable $X$ is measurable with respect to a generated sigma algebra, then there is a measurable function of the random variables generating the sigma algebra which is equal to $X$. We also have that $u_\varep = F_\varep(\zeta_{[t_0  - \varep, \infty)}) \stackrel{a.s.}{\ra} F(\zeta_{[t_0, \infty)}, \mc{N}) = u$. But since $\tilde{\zeta}$ has the same law as $\zeta$, we then have that $\tilde{u}_\varep = F_\varep(\tilde{\zeta}_{[t_0 - \varep, \infty)}) \stackrel{a.s.}{\ra} F(\tilde{\zeta}_{[t_0, \infty)}, \mc{N}) = F(\zeta_{[t_0, \infty)}, \mc{N}) = u$, as desired.}


% Here, $R_\varep = (G - K) \ast \zeta_\varep$.
% \todo{need to be careful about independence here, if we define $\Phi_\varep$ by smoothing in space-time.} \sky{Ok, I got confused by the following thing: in regularity structures, in principle we need to control the evaluation map $(\Pi_z \tau)[\varphi_z^\lambda]$ at points $z$ which possibly have negative time. This would be very problematic for us when we try to iterate, because the independence no longer holds at negative times. On the other hand, our use of the noise at negative times is really just a convenience, and in the end, the noise at negative times does not enter into the solution. Thus, as long as we assume that $u(t)$ is independent of the noise after time $t$ (which is certainly the case, since $u$ is adapted), our arguments can be made to work. Basically, at iteration step $j$, corresponding to a time $t_j$, we replace $\zeta$ by $\zeta^j + \zeta|_{[t_j, \infty)}$, where $\zeta^j$ is a white noise on $(-\infty, t_j] \times \T^2$, and independent of everything else. This modified noise is still a spacetime white noise on $\R \times \T^2$, and is moreover independent of $u(t_j)$, and thus also independent of the deterministic piece $\determ_j$ at time $t_j$.}
% \begin{equs}
% \sgnoiseplus{\determ_\varep, \varep} := e^{\icomplex \beta \determ_\varep} \biglcol\, e^{\icomplex \beta \Phi_\varep} \bigrcol, \quad \sgnoiseminus{\determ_\varep, \varep} := e^{-\icomplex \beta \determ_\varep} \biglcol \, e^{-\icomplex \beta \Phi_\varep} \bigrcol.
% \end{equs}
% \begin{equs}\label{eq:modified-noise}
% \xi_{\pm}^{\determ_\varep, \varep }:= e^{\pm \icomplex \beta \determ_\varep} \biglcol\, e^{\pm \icomplex \beta \Phi_\varep} \bigrcol = e^{\pm \icomplex \beta \determ_\varep} C_{\beta, \rho, \varep} e^{\pm \icomplex \beta \Phi_\varep},
% % \quad \xi_-^{\determ_\varep, \varep}:= e^{-\icomplex \beta \determ_\varep} \biglcol \, e^{-\icomplex \beta \Phi_\varep} \bigrcol.
% \end{equs}
% where we define the constant
% \begin{equs}\label{eq:gmc-renorm-constant}
% C_{\beta, \rho, \varep} := e^{\frac{\beta^2}{2} \E \Phi_\varep(0)^2}.
% \end{equs}


% In this section, we write out our Ansatz for the solution $u$ to \eqref{eq:SG}. \todo{introduce general time $t_0$} We write
% \begin{equs}
% u = \linear + \determ + v,
% \end{equs}
% where
% \begin{equs}
% \linear = \int_{-\infty}^t ds e^{(t-s)\Delta)} \xi(s),
% \end{equs}
% the deterministic piece $\determ$ satisfies the equation
% \begin{align}\label{eq:determ}
% \begin{split}
% (\ptl_t - \Delta) \determ &= \frac{\beta}{2} \int \dzprime K(\zprime; \cdot) \mc{J}^-(\zprime - \cdot) \sin\big(\beta(\determ(\cdot) - \determ(\zprime))\big), \\
% \determ(0) &= u_0. 
% \end{split}
% \end{align}
% \todo{check factor}
% and $v$ satisfies the equation
% \begin{equs}\label{eq:v-equation}
% (\ptl_t - \Delta) v &= \frac{1}{2\icomplex} \big( \sgnoiseplus{\determ} e^{\icomplex \beta v} - \sgnoiseminus{\determ} e^{-\icomplex \beta v}\big) - \frac{\beta}{2} \int \dzprime K(\zprime;\cdot) \mc{J}^-(\zprime - \cdot) \sin\big(\beta(\determ(\cdot) - \determ(\zprime))\big), \\
% v(0) &= -\linear(0). 
% \end{equs}
% \sky{If we are putting all the initial data $u_0$ in $\phi$, can we just assume that $v(0) = 0$? In other words, we can put $\phi(0) = u_0 - \linear(0)$.} \bjoern{I am not sure about that. Because if we do, then $\phi$ and $\linear$ will be probabilistically dependent?}
% Here, 
% \begin{equs}
% \sgnoiseplus{\determ} := e^{\icomplex \beta \determ} \biglcol\, e^{\icomplex \beta \linear} \bigrcol, \quad \sgnoiseminus{\determ} := e^{-\icomplex \beta \determ} \biglcol \, e^{-\icomplex \beta \linear} \bigrcol.
% \end{equs}
% To be more precise, we need to further split $v$ as follows. First, we define the ``dipoles" 
% \begin{equs}
% \todo{} &:= \sgnoiseplus{\determ} K \ast \sgnoiseminus{\determ} - \sgnoiseminus{\determ} K \ast \sgnoiseplus{\determ} - \int \dzprime K(\zprime; \cdot) \mc{J}^-(\zprime - \cdot) \sin\big(\beta(\determ(\cdot) - \determ(\zprime))\big), \\
% \todo{} &:= \sgnoiseplus{\determ} K \ast \sgnoiseplus{\determ}, \\
% \todo{} &:= \sgnoiseminus{\determ} K \ast \sgnoiseminus{\determ}.
% \end{equs}

% \todo{I think we need a terminilogy for $\sgnoiseplus{\determ}$ which separates it from the original object $\sgnoiseplus{}$ in Hairer-Shen. I.e. ``...." monopole/dipole/stochastic object etc. Is it maybe modified stochastic object? Conjugated stochastic object?...}


% We note that the initial value problem \eqref{eq:determ} can now be rewritten as 
% \begin{equation}\label{setup:eq-resonant-equation}
% (\partial_t - \Delta + m^2) \determ_\varep = \Res_\varep ( \determ_\varep ), \qquad \determ (0)=u_{0, \varep}. 
% \end{equation}
% In the following, we therefore refer to \eqref{eq:determ} or, equivalently, \eqref{setup:eq-resonant-equation}, as the resonant equation. 


% \bjoern{I think the exponent of $J$ should also depend on $\eta$. I guess we just assume that $\eta$ is small as well? I guess the precise power being close to $\frac{1}{2}$ doesn't really matter, since we got $J^{C_1}$ down below anyway.}\sky{I added $\eta$. Even in the local theory \cite{CHS2018} $\eta$ is always $\geq -1$, so $-\eta$ can be absorbed into $C_1$, as you say.}
% By taking $C_1$ sufficiently large depending on $C, c_0, \kappa$, and then by splitting into cases $\|u_0\|_{\Cs_x^{\eta}} > C_1 J^{C_1}/4$ and $\|u_0\|_{\Cs_x^{\eta}} \leq C_1 J^{C_1}/4$, we may further obtain
% \begin{equs}
% \|e^{c_0 t}  \determ_\varep\|_{C_t^0 \Cs_x^{\eta}([0, 1/J])}  \leq \max\Big(\frac{C_1}{2} J^{C_1}, e^{c_1/J} \|u_0\|_{\Cs_x^{\eta}}\Big) \leq \frac{C_1}{2} J^{C_1} + e^{c_1/J} \|u_0\|_{\Cs_x^{\eta}}.
% \end{equs}
% \bjoern{If  we just want the right-most term (and not the one in the middle), could it be easier to use the Young's inequality
% \begin{equs}
% C e^{c_0 / J} J^{-\frac{1}{2}(1-\kappa)} \|u_0\|_{\Cs_x^{\eta}}^{1-\kappa} 
% &= \big( c_1 J^{-1} \| u_0 \|_{\Cs_x^\eta} \big)^{1-\kappa} 
% \times c_1^{-(1-\kappa)} C e^{c_0 / J} J^{\frac{1}{2}(1-\kappa)}  \\ 
% &\leq c_1 J^{-1} \| u_0 \|_{\Cs_x^\eta} +  \big( c_1^{-(1-\kappa)} C e^{c_0 / J} J^{\frac{1}{2}(1-\kappa)} \big)^{\frac{1}{\kappa}}.
% \end{equs}
% Since our last project, I am always a bit concerned about switching between max and sums when constant factors matter.
% }


% \bjoern{Actually, I am a bit confused about this now. Did we really mean to derive the model from the pre-model? Because I think we also discussed just computing the pre-model from the first identity in Proposition \ref{appendix:prop-model-and-moments}?}

% \sky{My understanding was that we need to verify Proposition \ref{appendix:prop-model-and-moments} for our modified model. This would involve calculating the model obtained from our modified pre-model, and then checking that the formula matches with the one in the proposition.}
% \bjoern{Ok, then let me continue computing the expressions coming from Proposition \ref{appendix:prop-model-and-moments} first. I'll get on computing the model from the pre-model afterwards.}


% \section{Reconstruction using the modified model}\label{appendix:reconstruction}

% In this section, we prove Proposition \ref{prop:reconstruction}. 

% We define our model $(\Pi, \Gamma) = (\Pi^\phi, \Gamma^\phi)$ by
% \begin{equs}
% \Pi^\phi_z \Xi_+ = \sgnoiseplus, ~~ \Pi^\phi_z \Xi_- := \sgnoiseminus, 
% \end{equs}
% \begin{equs}
% \Pi^\phi_z (\Xi_+ \mc{I} \Xi_+) := \sgnoiseplus{} \big((K * \sgnoiseplus{}) - (K * \sgnoiseplus{})(z)\big), ~~ \Pi^\phi_z(\Xi_- \mc{I} \Xi_-) := \sgnoiseminus{} ((K * \sgnoiseminus{} - (K * \sgnoiseminus{})(z)), \label{eq:model-dipole-plus-plus-or-minus-minus} \\
% \Pi^\phi_z (\Xi_- \mc{I} \Xi_+) := \sgnoiseminus{} \big(K * \sgnoiseplus{} - (K * \sgnoiseplus{})(z)\big) - \int dw K(w - \cdot) \Jc^{-}(w - \cdot) e^{\icomplex \beta(\phi(w) - \phi(\cdot))}, \\
% \Pi^\phi_z (\Xi_+ \mc{I} \Xi_-) := \sgnoiseplus{} \big(K * \sgnoiseminus{} - (K * \sgnoiseminus{})(z)\big) - \int dw K(w - \cdot) \Jc^{-}(w - \cdot) e^{-\icomplex \beta(\phi(w) - \phi(\cdot))}.
% \end{equs}
% \begin{equs}

% \end{equs}
% \bjoern{Stupid question: What exactly are the consistency questions which our definitions of $\Pi^\phi_z (\textup{tripoles})$ need to satisfy, given that we fixed that for the monopoles and dipoles? Clearly, they have to be related somehow? In the canonical (non-renormalized) model, the one for the tripole is of course defined by the one for the monopole. But how much/in what way can we change that?}\\
% \sky{As far as I understand, in the abstract theory, one only requires the model to be admissible, i.e. $\Pi_x \tau$ must have homogeneity $\mrm{deg} \tau$, the recentering $\Gamma_{xy}$ must respect homogeneity in the natural way, and $\Pi_x$ must interact with $\mc{I}$ nicely. Nothing is imposed about products of symbols. In practical situations, we need to ensure that (a) the model converges (b) reconstruction gives the right PDE.}\\
% \bjoern{Ok, so then I am still confused about this. Which of these then stops me from simply setting, for all $w,z$, 
% \begin{equation*}
% \Pi_z\big( \Xi_{s_1} \mc{I} \Xi_{s_2} \mc{I} \Xi_{s_3})(w) = 0 
% \qquad \text{and} \qquad 
% \Gamma_{wz} \big( \Xi_{s_1} \mc{I} \Xi_{s_2} \mc{I} \Xi_{s_3}) = \Xi_{s_1} \mc{I} \Xi_{s_2} \mc{I} \Xi_{s_3}?
% \end{equation*}
% At least on the linear space spanned by $\Xi_{s_1} \mc{I} \Xi_{s_2} \mc{I} \Xi_{s_3}$, all the algebraic identities and estimates needed for the model $(\Pi,\Gamma)$ are satisfied. And $\Xi_{s_1} \mc{I} \Xi_{s_2} \mc{I} \Xi_{s_3}$ itself is not an integral, so I am not sure how the constraints from $\mc{I}$ would enter here. And I don't think this definition can be allowed, since otherwise the proof for $\beta^2<6\pi$ would be the same as for $\beta^2<\frac{16\pi}{3}$. 
% What am I missing?
% }\\
% \bjoern{Actually, I  was just thinking: What about the notion of $\gamma$-regular sectors from \cite[Definition 4.6]{H14}? Does this pose some restriction of how $\Gamma_{xy}$ acts on products?} \\
% \sky{Yes, I think the definition of $\Gamma$ is imposed from certain constraints -- see the discussion around the middle of page 118 of \cite{H14}, as well as equation (5.19) of the paper. Although, I see your point, and I'm not yet sure what goes wrong if we just set $\Pi (\mrm{tripole}) = 0$ (of course, I agree something should go wrong).} \\
% \sky{Ok, if $\Gamma$ is multiplicative and $\Gamma \Xi_{\pm} = \Xi_{\pm}$, then in order to have 
% \begin{equs}
% \Pi_x \Gamma_{xy} (\Xi_- \mc{I} \Xi_+) = \Pi_y (\Xi_- \mc{I} \Xi_+),
% \end{equs}
% we are forced to set
% \begin{equs}
% \Gamma_{xy} (\mc{I} \Xi_+) = \mc{I} \Xi_+ + ((K * \sgnoiseplus{})(x) - (K * \sgnoiseplus{})(y)) \mbf{1}.
% \end{equs}
% From this, we then have that
% \begin{equs}
% \Gamma_{xy} (\Xi_- \mc{I} \Xi_+ \mc{I} \Xi_+) &= \Xi_- \big(\mc{I} \Xi_+ + ((K * \sgnoiseplus{})(x) - (K * \sgnoiseplus{})(y)) \mbf{1}\big)^2 \\
% &= \Xi_- \mc{I} \Xi_+ \mc{I} \Xi_+ + 2 ((K * \sgnoiseplus{})(x) - (K * \sgnoiseplus{})(y)) \Xi_- \mc{I} \Xi_+ + \Xi_- ((K * \sgnoiseplus{})(x) - (K * \sgnoiseplus{})(y))^2.
% \end{equs}
% This is where some constraint on $\Pi(\mrm{tripole})$ enters, since we need to ensure that $\Pi_x \Gamma_{xy} = \Pi_y$. If we define
% \begin{equs}
% \Pi_x (\Xi_- \mc{I} \Xi_+ \mc{I} \Xi_+) = \sgnoiseminus{} (K * \sgnoiseplus{} - (K * \sgnoiseplus{})(x)) - 2 \E[\sgnoiseminus{} (K * \sgnoiseplus{})] (K * \sgnoiseplus{} - (K * \sgnoiseplus{})(x)),
% \end{equs}
% then the relation is satisfied.
% }



% Let $\mu \in (\frac{\beta^2}{4\pi}, 2)$. 

% \sky{I am confused about the following point: do we need to add a projection in front of the integration operator $\mc{P}$? Since $W \in \mc{D}_0^{\mu, 0}$, its expansion only has elements of homogeneity up to $\mu$. However, one of the terms appearing on the right hand side is an integrated tripole, which has homogeneity $6 - \frac{3\beta^2}{4\pi} > \mu$ (assuming $\mu$ is chosen close enough to $\beta^2 / 4\pi$).}


% Consider the following fixed point problem for $V \in \mc{D}^{\mu}_0$:
% \begin{equation}\label{eq:regularity-structures-fixed-pt=problem}
% V = (\mc{K}_\mu + R_\mu \mc{R}) \mathbf{R}^+ F(V) + G v_0.
% \end{equation}

% \begin{lemma}
% Let $0 < \beta^2 < 6\pi$. With the model $(\Pi, \Gamma)$ defined as in \todo{}, we have that the reconstruction $v = \mc{R} V$ satisfies \eqref{eq:v-equation}.
% \end{lemma}
% \begin{proof}
% Applying the reconstruction operator $\mc{R}$ to both sides of \eqref{eq:regularity-structures-fixed-pt=problem}, we get that
% \[ \mc{R} V = (K + R) \mc{R} F(V) + G v_0 = G \mc{R} F(V) + G v_0,\]
% and it remains to verify that $\mc{R} F(V) = F(\mc{R} V)$. Since $V \in \mc{D}_0^\mu$, and since $V$ solves \eqref{eq:regularity-structures-fixed-pt=problem}, we have the following expansion for $V$ \todo{maybe add more detail. It may make more sense to put this after the expansion of $e^{\pm \icomplex \beta V}$, because that expansion is where this ansatz comes from}:
% \begin{equs}
% V = f_0 \mbf{1} + f_1 X_1 + f_2 X_2 + \frac{1}{2\icomplex} \big( e^{\icomplex \beta f_0} \mc{I} \Xi_+ - e^{-\icomplex \beta f_0} \mc{I} \Xi_-\big) &+ \frac{\beta}{4\icomplex} \big(e^{\icomplex 2 \beta f_0} \mc{I}(\Xi_+ \mc{I} \Xi_+) - e^{-\icomplex 2 \beta f_0} \mc{I}(\Xi_- \mc{I} \Xi_-)\big) \\
% &+ \frac{\beta}{4\icomplex} \big(\mc{I}(\Xi_- \mc{I} \Xi_+) - \mc{I}(\Xi_+ \mc{I} \Xi_-)\big).
% \end{equs}
% Note that $\mc{R} V = f_0$. Let $\tilde{V} = V - f_0 \mbf{1}$. We have that
% \begin{equs}
% e^{\icomplex \beta V} &= e^{\icomplex \beta f_0}\bigg(\mbf{1} + \icomplex \beta \tilde{V} + \frac{(\icomplex \beta)^2}{2} \tilde{V}^2\bigg), \\
% e^{-\icomplex \beta V} &= e^{-\icomplex \beta f_0}\bigg(\mbf{1} - \icomplex \beta \tilde{V} + \frac{(-\icomplex \beta)^2}{2} \tilde{V}^2 \bigg),
% \end{equs}
% % where $\eta_+, \eta_- \in \mc{D}^\mu_{3(2 - \frac{\beta^2}{4\pi})}$ are higher-homogeneity remainders.
% where we used that $\beta^2 < 6\pi$ so that the high-homogeneity remainders (which have minimum homogeneity $3(\beta^2 - 4\pi)$) do not appear upon projecting to $\mc{T}_{< \mu}$. \todo{we need to specify that $\mu$ is chosen close to $\beta^2 / 4\pi$ depending on how close $\beta^2$ is to $6\pi$.} Inserting these expansions, we obtain
% \begin{equs}
% F(V) = \frac{1}{2\icomplex} \big(e^{\icomplex\beta f_0} \Xi_+ - e^{-\icomplex \beta f_0} \Xi_-\big) &+ \frac{\beta}{2} \tilde{V} (e^{\icomplex \beta f_0} \Xi_+ + e^{-\icomplex \beta f_0}\Xi_-) \\
% &- \frac{\beta^2}{4\icomplex} \tilde{V}^2 \big(e^{\icomplex \beta f_0} \Xi_+ - e^{-\icomplex \beta f_0} \Xi_-\big).
% \end{equs}
% The desired result follows from the following three claims.
% \begin{align}
% \frac{1}{2\icomplex} \mc{R} \Big(\big(e^{\icomplex\beta f_0} \Xi_+ - e^{-\icomplex \beta f_0} \Xi_-\big)\Big) &= \frac{1}{2}\big( e^{\icomplex \beta f_0} \sgnoiseplus{} - e^{-\icomplex \beta f_0} \sgnoiseminus{} \big), \label{eq:reconstruction-intermediate-1} \\
% \frac{\beta}{2} \mc{R} \Big( \tilde{V} (e^{\icomplex \beta f_0} \Xi_+ + e^{-\icomplex \beta f_0}\Xi_-) \Big) &= \frac{\beta}{4\icomplex} \Pi_x \Big(\mc{I}\big(\Xi_- \mc{I} \Xi_+\big) - \mc{I}\big(\Xi_+ \mc{I} \Xi_-\big) \Big)(x) = -\Res(\phi) , \label{eq:reconstruction-intermediate-2} \\
% \mc{R} \Big(\tilde{V}^2 \big(e^{\icomplex \beta f_0} \Xi_+ - e^{-\icomplex \beta f_0} \Xi_-\big)\Big) &= 0.\label{eq:reconstruction-intermediate-3}
% \end{align}
% Note that the second identity in \eqref{eq:reconstruction-intermediate-2} follows from \eqref{eq:dipole-resonance}.
% The first identity \eqref{eq:reconstruction-intermediate-1} follows immediately from the definition of $\mc{R}$. To check the second identity \eqref{eq:reconstruction-intermediate-2}, we note that for $j \in [2]$, we have that $\mc{R}(X_j \Xi_{\pm}) = 0$ by construction. We will show that
% \begin{align}
% \mc{R} \Big( \big( e^{\icomplex \beta f_0} \mc{I} \Xi_+ - e^{-\icomplex \beta f_0} \mc{I} \Xi_-\big) (e^{\icomplex \beta f_0} \Xi_+ + e^{-\icomplex \beta f_0} \Xi_-) \Big) &= \Pi_z \Big(\mc{I}\big(\Xi_- \mc{I} \Xi_+\big) - \mc{I}\big(\Xi_+ \mc{I} \Xi_-\big) \Big)(z), \label{eq:dipole-reconstruction}\\
% \mc{R} \Big( \big(\mc{I}(\Xi_- \mc{I} \Xi_+) - \mc{I}(\Xi_+ \mc{I} \Xi_-)\big) (e^{\icomplex \beta f_0} \Xi_+ + e^{-\icomplex \beta f_0} \Xi_-)\Big) &= 0. \label{eq:line-tripole-reconstruction}
% \end{align}
% The second identity \eqref{eq:reconstruction-intermediate-2} will then follow by combining these identities. We note that \eqref{eq:dipole-reconstruction} follows immediately from the construction of $\Pi$, in particular from \eqref{eq:model-dipole-plus-plus-or-minus-minus}, we have that
% \begin{equs}
% \Pi_z(\Xi_+ \mc{I} \Xi_+)(z) = \Pi_z(\Xi_- \mc{I} \Xi_-)(z) &= 0.
% % \Pi_z(\Xi_- \mc{I} \Xi_+)(z) &= \int \dw e^{\icomplex \beta (\phi(w) - \phi(z)} K(w - z) \Jc^-(w - z) , \\
% % \Pi_z(\Xi_+ \mc{I} \Xi_-)(z) &= \int \dw e^{-\icomplex \beta (\phi(w) - \phi(z)} K(w - z) \Jc^-(w - z).
% \end{equs}
% The identity \eqref{eq:line-tripole-reconstruction} follows by.
% % Finally, to verify \eqref{eq:reconstruction-intermediate-3}, again note that upon expanding $\tilde{V}^2$, any term with a polynomial term is sent to zero $\mc{R}$. Then by homogenity counting, and using that $\beta^2 < 6\pi$, we see that the only term which has negative homogeneity is (ignoring a $(1/2i)^2$ prefactor)
% % \begin{equs}
% % \big( e^{\icomplex \beta f_0} \mc{I} \Xi_+ - e^{-\icomplex \beta f_0} \mc{I} \Xi_-\big)^2 \big( e^{\icomplex \beta f_0} \Xi_+ - e^{-\icomplex \beta f_0} \Xi_-\big) .
% % \end{equs}
% % To finish, recall that for any $s_1, s_2, s_3 \in \{\pm\}$, we have by \todo{verify that tripole is fine} that for any $z$,
% % \begin{equs}
% % \Pi_z\big( \Xi_{s_1} \mc{I} \Xi_{s_2} \mc{I} \Xi_{s_3})(z) = 0.
% % \end{equs}
% \end{proof}
